Block-distributed Gradient Boosted Trees

The Gradient Boosted Tree (GBT) algorithm is one of the most popular machine learning algorithms used in production, for tasks that include Click-Through Rate (CTR) prediction and learning-to-rank. To deal with the massive datasets available today, many distributed GBT methods have been proposed. However, they all assume a row-distributed dataset, addressing scalability only with respect to the number of data points and not the number of features, and increasing communication cost for high-dimensional data. In order to allow for scalability across both the data point and feature dimensions, and reduce communication cost, we propose block-distributed GBTs. We achieve communication efficiency by making full use of the data sparsity and adapting the Quickscorer algorithm to the block-distributed setting. We evaluate our approach using datasets with millions of features, and demonstrate that we are able to achieve multiple orders of magnitude reduction in communication cost for sparse data, with no loss in accuracy, while providing a more scalable design. As a result, we are able to reduce the training time for high-dimensional data, and allow more cost-effective scale-out without the need for expensive network communication.

==> related.tex <==
Due to the wide adoption of GBTs, there have been multiple attempts
to optimize their performance and train on massive, distributed
datasets. One of the most popular GBT algorithms
is XGBoost \cite{xgboost} which focused on improving the performance
of parallel tree learning using out-of-core computation, cache-aware
algorithms, and sparsity-aware histogram construction.
The popularity of XGBoost sparked further research into distributed GBT
systems. LightGBM \cite{lightgbm} made use of the scatter-reduce communication
pattern to improve the communication cost of histogram construction, along
with a communication-efficient split selection algorithm \cite{comm-efficient-gbt}.
Finally, DimBoost \cite{dimboost} was the first paper to use the parameter server
for GBTs and brought a number of improvements,
such as gradient compression, and a load-balanced split selection algorithm,
however it also uses row distribution and dense communication.

Prior attempts at distributing the training along the feature dimension
assumed that the complete dataset would fit in the main
memory of each worker \cite{lightgbm, xgboost}.

